Dordis: Efficient Federated Learning with Dropout-Resilient Differential Privacy

Federated learning (FL) is increasingly deployed among multiple clients to train a shared model over decentralized data. To address privacy concerns, FL systems need to safeguard the clients' data from disclosure during training and control data leakage through trained models when exposed to untrusted domains. Distributed differential privacy (DP) offers an appealing solution in this regard as it achieves a balanced tradeoff between privacy and utility without a trusted server. However, existing distributed DP mechanisms are impractical in the presence of client dropout, resulting in poor privacy guarantees or degraded training accuracy. In addition, these mechanisms suffer from severe efficiency issues. We present Dordis, a distributed differentially private FL framework that is highly efficient and resilient to client dropout. Specifically, we develop a novel `add-then-remove' scheme that enforces a required noise level precisely in each training round, even if some sampled clients drop out. This ensures that the privacy budget is utilized prudently, despite unpredictable client dynamics. To boost performance, Dordis operates as a distributed parallel architecture via encapsulating the communication and computation operations into stages. It automatically divides the global model aggregation into several chunk-aggregation tasks and pipelines them for optimal speedup. Large-scale deployment evaluations demonstrate that Dordis efficiently handles client dropout in various realistic FL scenarios, achieving the optimal privacy-utility tradeoff and accelerating training by up to 2.4$\times$ compared to existing solutions.

==> content/accounting.tex <==
%!TEX root = ../main.tex
\section{Dropout-Resilient Privacy Accounting}
\label{sec:accounting}

We design a new privacy accounting approach for a tight analysis of
privacy loss subject to client dropout before sampling. We then use it to
determine the minimum noise required in each training round to control data
leakage within the privacy budget. Our approach is built on the notion of 
R{\'e}nyi DP.

% We start with \emph
% {facts} necessary for the reader to understand the technical details.

\PHM{A Primer on R{\'e}nyi DP.} R{\'e}nyi DP~\cite{mironov2017renyi} is an
 alternative DP notion that gives a tighter privacy analysis than the
 traditional $(\epsilon, \delta)$-DP. Recall in Equation~\eqref{eq:dp} that
 $(\epsilon, \delta)$-DP bounds the $\delta$-approximate max-divergence~\cite{max-divergence} in the output
 distribution of a randomized algorithm subject to a small
 change in input. R\'enyi DP, expressed with two parameters $(\alpha, \epsilon)$, 
 upper-bounds the output's \emph
 {R\'enyi divergence} -- a measure of distance between two
 distributions -- by a small $\epsilon$ when the training set differs
 only in the inclusion of a single client's data, i.e., 
 $\textrm{R\'enyiDivergence}_\alpha(f(D),f
 (D')) \leq \epsilon$, where $\alpha > 1$ is a parameter of R\'enyi divergence.
 
R\'enyi DP has two important properties, which we briefly describe
while giving the math details in Appendix~\ref{sec:appendix_rdp}.

% \vspace*{-0.1in}

\begin{enumerate}[nosep]
    \item For every value of $\alpha$, there is a \emph{direct translation} from R\'enyi DP to $(\epsilon, \delta)$-DP: $(\alpha, \epsilon-\frac{\log(1/\delta)}{\alpha-1})$-R\'enyi DP implies $(\epsilon, \delta)$-DP for any value of $\epsilon>0$, $\delta \in (0,1]$, and $\alpha>1$.
    This means that \system{} can use R\'enyi DP internally while exposing the same $(\epsilon, \delta)$-DP guarantee externally.
    \item Like $(\epsilon, \delta)$-DP, R\'enyi DP can also be \emph{additively composed}. That is, running an $(\alpha, \epsilon_1)$-R\'enyi DP and an $(\alpha, \epsilon_2)$-R\'enyi DP computation on the same dataset is $(\alpha, \epsilon_1 + \epsilon_2)$-R\'enyi DP.
    Yet, when translated to $(\epsilon, \delta)$-DP, the privacy loss accounted with R\'enyi DP is usually \emph{tighter} (i.e., sublinear) than that derived directly with $(\epsilon, \delta)$-DP, as R\'enyi DP utilizes the properties of the used DP mechanism (which affects the particular relationship between $\epsilon$ and $\alpha$, denoted by $\epsilon(\alpha)$), while $(\epsilon, \delta)$-DP does not.
\end{enumerate}

% \vspace*{-0.1in}

\PHM{Privacy Accounting in FL.}
Privacy accounting plays a key role in determining the minimum required noise
that should be added in each training round. Figure~\ref{fig:noise_privacy} shows 
how privacy accounting in FL can be done in three steps:

\begin{figure}[t]
    \centering
    \includegraphics[width=1\columnwidth]{./images/noise-privacy.eps}
    \caption{The procedure of privacy accounting in FL.}
    \label{fig:noise_privacy}
    \vspace*{-0.05in}
\end{figure}

% \vspace*{-0.05in}

\begin{enumerate}[nosep]
    \item Given a noise level (parameterized by the variance $\sigma^2$) and the client sampling rate, compute the privacy loss in the notion of R{\'e}nyi DP for one training round.
    \item Given the target number of training rounds, compute the cumulative privacy loss 
    using the composition theory.
    \item Translate the privacy loss expressed in R{\'e}nyi DP into the 
    traditional notion of $(\epsilon, \delta)$-DP.
\end{enumerate}

Among all three steps, the main challenge lies in Step 1, as the standard
theoretical tool used in privacy accounting (i.e., privacy amplification via subsampling~\cite
{zhu2019poission, wang2019subsampled}) assumes uniform client sampling, which
is not the case in FL given that clients can drop out before the sampling
takes place (\cref{sec:issue_client_dropout}).

\PHM{Dropout-Resilient Privacy Accounting.}
We develop a new theoretical tool for privacy accounting in Step 1 without
assuming the uniform sampling. In particular, we consider a \emph
{heterogeneous} sampling process in which clients are sampled
independently with non-uniform probabilities ranging from 0 to $\gamma < 1$. 
More formally, we have the following definition:

% As a by-product, it also accounts for \emph
% {other possible sources of randomness}, e.g., probabilistic hardware
% failures, that pulls down a client's actual participation rate below the
% target sampling probability.

\begin{definition}[\textup{\texttt{HeteroPoissonSample}}]
     Given a client set $C$ and the sampling probability bound $\gamma \in [0, 1)$, the process \textup{\texttt{HeteroPoissonSample}}$(C, \gamma)$ outputs a subset of clients $\{c_i \in C \mid \xi_i = 1\}$ by sampling $\xi_i \sim \text{Bernoulli}(\gamma_i)$, where $\gamma_i \in [0, \gamma]$.
    \label{def:heteropoissonsample}
\end{definition}

This \textup{\texttt{HeteroPoissonSample}} process captures the scenario where
clients are uniformly sampled with probability $\gamma$ but some may drop out
before sampling. For those dropped clients, their sampling rate is 0
(i.e., $\gamma_i = 0$). 

We next bound the privacy loss in the above sampling process. Intuitively, the
privacy loss reaches the maximum when clients are uniformly sampled with
probability $\gamma$. This is because having a client with less chance of
being sampled (i.e., $\gamma_i < \gamma$) should neither increase the data
exposure of its own nor the others'. Following this intuition, we derive a
tight bound of the privacy loss in \textup{\texttt{HeteroPoissonSample}} with
the following theorem, which generalizes the result of uniform sampling
(i.e., Theorem 5 in~\cite{zhu2019poission}) in a non-trivial way:

\begin{theorem}
    Let $f$ be a perturbation algorithm that is $(\alpha, \epsilon(\alpha))$-R{\'e}nyi DP and $g$ be the function composition $f(\textup{\texttt{HeteroPoissonSample}}(C, \gamma))$.
    For any integer $\alpha \geq 2$, the privacy loss of $g$ is tightly bounded by
    {\small
    \begin{align}
        \epsilon_{g}(\alpha)
        &\leq \frac{1}{\alpha - 1} \log \Biggl\{ (1-\gamma)^{\alpha - 1}(\alpha\gamma - \gamma + 1)
        + \binom{\alpha}{2} \gamma^2(1-\gamma)^{\alpha-2} e^{\epsilon(2)} \nonumber \\
        &+ 3 \sum_{l=3}^{\alpha} \binom{\alpha}{l} (1-\gamma)^{\alpha - l} \gamma^l e^{(l-1)\epsilon(l)} \Biggr\}.
        \label{eq:heteropoisson_rdp}
    \end{align}
    }%
    \label{thm:heteropoissonsample}
\end{theorem}
\vspace*{-0.15in}
For ease of notation, we denote the right-hand side of the above inequality~\eqref{eq:heteropoisson_rdp}, i.e., the upper bound, as $F(\gamma)$.
We give a proof sketch and refer to Appendix~\ref{sec:appendix_hetero} for the complete proof.

\begin{proofsketch}
Recall that R{\'e}nyi DP bounds the R{\'e}nyi divergence between the output distributions with and without a client $i$'s participation, namely $g(D_{i})$ and $g(D_{-i})$.
Our goal is to prove that $\textrm{R\'enyiDivergence}_\alpha(g(D_i),g(D_{-i})) \leq F(\gamma)$ and $\textrm{R\'enyiDivergence}_\alpha(g(D_{-i}),g(D_{i})) \leq F(\gamma)$ for any $i$.

The key to our proof (see Appendix~\ref{sec:appendix_hetero}) is to show that $F(\cdot)$ monotonically decreases. We therefore
have $F(\gamma_i) \leq F(\gamma)$ for all $\gamma_i \le \gamma$.
Combining this monotonicity with the fact 
that $\textrm{R\'enyiDivergence}_\alpha(g(D_i),g(D_{-i})) \leq F(\gamma_i)$ and $\textrm{R\'enyiDivergence}_\alpha(g(D_{-i}),g(D_{i})) \leq F(\gamma_i)$ for any client $i$ (established by Theorem 5 in~\cite{zhu2019poission}), we show that Equation~\eqref{eq:heteropoisson_rdp} holds
and conclude the proof.
\end{proofsketch}

Theorem~\ref{thm:heteropoissonsample} enables a tight analysis of privacy loss
at a certain noise level in one round without worrying about client dropout
before sampling, thereby facilitating the aforementioned Step 1 of privacy accounting in FL (Figure~\ref{fig:noise_privacy}). Following the remaining accounting procedure
(Steps 2 and 3), \system{} accounts the cumulative privacy loss
throughout training when a certain noise level is enforced in each round.
This essentially
enables \emph{offline noise planning} before the training starts (\cref{sec:background_dp}), in which
\system{} searches the minimum noise required, denoted by $\sigma^2_*$, in each of the $T$ training rounds subject
to a global privacy budget $(\epsilon_G, \delta_G)$ by solving

\vspace*{-0.05in}
{\small
\begin{align}
    \sigma^2_* &= \argmin_{\sigma^2} 
    \left\lVert \textup{RDP2DP}(T \cdot F(\gamma), \delta_G) - \epsilon_G \right\rVert,
    \label{eq:noise_privacy}
\end{align}
}where $\textup{RDP2DP}(x, y)$ translates a R\'enyi DP bound $x$ to a bound on $\epsilon$ in the $(\epsilon, \delta)$-DP notion, given that $\delta=y$.

